Optimizing pre-scheduled, intermittently-observed MDPs

A challenging category of robotics problems arises when sensing incurs substantial costs. This paper examines settings in which a robot wishes to limit its observations of state, for instance, motivated by specific considerations of energy management, stealth, or implicit coordination. We formulate the problem of planning under uncertainty when the robot's observations are intermittent but their timing is known via a pre-declared schedule. After having established the appropriate notion of an optimal policy for such settings, we tackle the problem of joint optimization of the cumulative execution cost and the number of state observations, both in expectation under discounts. To approach this multi-objective optimization problem, we introduce an algorithm that can identify the Pareto front for a class of schedules that are advantageous in the discounted setting. The algorithm proceeds in an accumulative fashion, prepending additions to a working set of schedules and then computing incremental changes to the value functions. Because full exhaustive construction becomes computationally prohibitive for moderate-sized problems, we propose a filtering approach to prune the working set. Empirical results demonstrate that this filtering is effective at reducing computation while incurring only negligible reduction in quality. In summarizing our findings, we provide a characterization of the run-time vs quality trade-off involved.

==> junkyard.tex <==
\subsection{Schedule costs}
In order to compare different schedules and their respective \psmdps, we must quantify the quality of each schedule in some manner. For any given schedule, we have its \psmdp which we can solve to obtain its value function $U^\ast(s)$ and optimal policy $\pi^\ast$. The value function signifies the expected discounted cumulative cost to reach the goal state from a certain state---we can define the \textit{execution cost} for a schedule as the expected cost over the initial distribution of start states.

\begin{definition}
For a schedule $\sched$, initial distribution $S_0$, and value function $U^\ast(s)$, the \emph{execution cost} of the schedule is
$$\mathbf{E}(\sched) = \sum_{s \in S_0} U^\ast(s) \Pr(s)$$
\end{definition}

Similarly, we can define a \textit{check-in cost} equal to the expected number of check-ins needed over the initial distribution to reach the goal state. As each check-in directly corresponds to an action sequence in the \psmdp, the check-in cost is the same as the expected hitting time of the \psmdp.

\begin{definition}
For a schedule $\sched$, initial distribution $S_0$, and expected hitting times $H(s)$, the \emph{check-in cost} of the schedule is
$$\mathbf{C}(\sched) = \sum_{s \in S_0} H(s) \Pr(s)$$
\end{definition}

\textcolor{orange}{I don't think this is right, as you need more nuance with time. In \eqref{eqn:cost-seq-discount}, there is a time index $t$; this is the sole place where \emph{time} as a concept is employed. Instead, you need to use $\idx{\hat{t}}$, where $\hat{t}$ is the time, in the sense of steps of clock $t$ to determine the number of check-ins. I \textit{think} this is right, but we need to tred carefully here, and make sure what I said is true, and that you can apply the function to an expectation.}



For initial state distribution $\InitD : S \to [0,1]$,
the traditional performance measure 
for a robot executing a sequence of actions is
the \emph{expected discounted cumulative cost} to a goal:
%\begin{equation}
%V(\InitD)=\expectation{\sum_{\dt=0}^{\infty} \gamma^{\dt} C\left(s^{\dt},a^{\dt}\right)},\text{ with } s^{0} \sim \InitD,
%\label{eqn:cost-seq-discount}
%\end{equation}
with the expectation ranging over state sequences, $s^0, s^1, \dots, s^\tau$, that arrive at some $s^\tau \in G$,
starting from some $s^{0}$ drawn according to $\InitD$,
and following the transition dynamics given the actions $a^{0}, a^{1}, a^{2}, \dots$. 

\begin{definition}[bounded stride]
Schedule $\sched$ has \emph{stride bounded by $\strideBound$} if \mbox{$\sched(n) \leq \strideBound$} for all $n \in \Nats$.
\end{definition}

\begin{definition}[tail recurrent]
Some schedule $\sched$ is said to be \emph{tail recurrent} if there exists some $N_0 \in \Nats$ such that 
\mbox{$\sched(n+1) = \sched(n)$} for all $n \geq N_0$.
\end{definition}


All subsequent illustrative examples will have stride bounded by $\strideBound \leq 9$, 
so schedules such as $\seq{1\sS 3\sS 2\sS 1\sS 3\sS \recc{2}}$ can 
save ink by being given 
more sleekly as just $13213\recc{2}$.

\begin{proposition}
\label{prop:opt-exists}
Given \psmdp $\langle S, A, T, \costC, G, \sched \rangle$ 
and initial state distribution $\InitD$,
a stationary and deterministic \psmdp policy 
$\optPi : S \times \Nats \to A^\infty$
always exists that minimizes the expected discounted cumulative cost 
 to $G$
\begin{equation}
%V_\pi(\InitD)=
\expectation{\sum_{\dt=0}^{\infty} \gamma^{\dt} C\left(s^{\dt},a^{\dt}\right)},
\label{eqn:cost-seq-discount}
\end{equation}
with the expectation ranging over state sequences, $s^0, s^1, \dots,
s^\tau$, that arrive at some $s^\tau \in G$, starting from some $s^{0}$ drawn
according to $\InitD$, and following the transition dynamics given the actions
$a^{0}, a^{1}, a^{2}, \dots, a^{\tau-1}$. 
The minimization is across all prescriptions for actions which access state
only at times in the schedule:
\scalebox{0.93}{% 
$\seq{0\sS  \sched(0)\sS \allowbreak \sched(0)\!+\!\sched(1)\sS \sched(0)\!+\!\sched(1)\!+\!\sched(2)\sS  \dots\sS  \sum_{i=0}^{m-1} \sched(i)\sS  \dots}$%
}.
\end{proposition}

\textcolor{red}{
TODO: Re-write this as a $\min$ and $\arg\min$ over all 
$V_{\pi}(\InitD;\mathcal{M})$ for \psmdp policies. Denote that 
$V^\opt_{\pi}(\InitD;\mathcal{M})$ for \psmdp policies. 
}

%In this paper, we consider a two phase interaction:
%firstly, one agent, the \emph{\observer}, is responsible for choosing 
%a schedule and declaring that to the \psmdp system. Operationally, the agent will then generate
%check-ins while being faithful to that schedule. The 
%\psmdp system, or \emph{\actor},  will then seek to minimize the expected cost of its execution for
%the given schedule of check-ins; the \actor will, thus, obtain a
%$\vect{\pi}$ and execute that. As the agents are interested in minimizing different quantities, they must negotiate in order to determine a schedule and a policy that is suitable for both of them. 
%
%(An alternative model, which we will not pursue here, is where the two agents negotiate to determine the schedule.)
%
%In this paper, we consider a two phase interaction:
%firstly, one agent, the \emph{\observer}, is responsible for choosing 
%a schedule and declaring that to the \psmdp system. Operationally, the agent will then generate
%check-ins while being faithful to that schedule. The 
%\psmdp system, or \emph{\actor},  will then seek to minimize the expected cost of its execution for
%the given scheduled of check-ins; the \actor will, thus, obtain a
%$\vect{\pi}^\opt$ and execute that. 
%(An alternative model, which we will not pursue here, is where the two agents negotiate to determine the schedule.)
%
%\subsection{Schedule Costs}
%

To show that above notion is indeed appropriate for \psmdps, 
we will present Proposition~\ref{prop:opt-exists}; first 
we need the following two definitions, defining a sort of unwinding\gobble{ across time}:

\begin{definition}[Transition Composition~\cite{rossi22periodic}]
\label{defn:t-composition}
For some $k \in \Nats$ and transitions $T: S\times A \times S \to [0,1]$, the
\emph{$k$-composed transition model} is the function $T^k: S\times A^k \times S \to [0,1]$ defined as

\vspace*{-4ex}
%\vspace*{-1ex}
{\small
\begin{equation*}
T^{k}\left(s',(a_0, \dots, a_{k-1}), s\right)  = \!\!\!\!\!\!\!\!\!\sum_{\substack{(s_0, \dots, s_{k-1})\in S^k\\ \text{where } s_0 = s\\ \text{ and } s_{k} = s'}} \prod_{i=0}^{k-1} T(s_{i+1},a_i,s_i).
\end{equation*}
}
\end{definition}

\begin{definition}[Cost Composition~\cite{rossi22periodic}]
\label{defn:costcompositions}
For discounting factor $\gamma \in (0,1)$ and cost
function $C: S\times A\to \Reals$, the \emph{macro $\gamma$-discounted cost} is
the function $\vect{C}^{\gamma}: S\times A^\infty \to\Reals$ defined as
\vspace*{-2.3ex}
{\small
%\begin{align*}
$$
\vect{C}^{\gamma}\left(s,\vec{a}\right) = \vect{C}^{\gamma}\left(s,(a_0, a_1, \dots a_{k-1})\right) = \nonumber \\[-2pt]
%\hspace*{10ex}
\sum_{m = 0}^{k-1} \;\;\;\, \gamma^{\verythinspace m}\!\!\!\!\!\!\!\!\!\!\!\! \sum_{\substack{(s_0, \dots, s_{m})\in S^{m+1}\\ \!\!\!\text{where } s_0 = s}} \!\!\!\!\!\!\!\!C(s_{m}, a_{m}) \prod_{i=0}^{m-1} T(s_{i+1},a_i,s_i).
%\end{align*}
$$
}
\end{definition}




\begin{definition}[Cost Composition~\cite{rossi22periodic}]
\label{defn:costcompositions}
For some $k \in \Nats$, discounting factor $\gamma \in (0,1)$, and cost
function $C: S\times A\to \Reals$, the \emph{$k$-composed $\gamma$-discounted cost} is
the function $C^{k,\gamma}: S\times A^k \to\Reals$ defined as

\vspace*{-2.3ex}
{\small
\begin{align*}
&C^{k,\gamma}\left(s,\vec{a}\right) = C^{k,\gamma}\left(s,(a_0, a_1, \dots a_{k-1})\right) = \nonumber \\[-2pt]
&\hspace*{10ex}\sum_{m = 0}^{k-1} \;\;\;\, \gamma^{\verythinspace m}\!\!\!\!\!\!\!\!\!\!\!\! \sum_{\substack{(s_0, \dots, s_{m})\in S^{m+1}\\ \!\!\!\text{where } s_0 = s}} \!\!\!\!\!\!\!\!C(s_{m}, a_{m}) \prod_{i=0}^{m-1} T(s_{i+1},a_i,s_i).
\end{align*}
}
\end{definition}



\textcolor{red}{We should provide some intuition; notice that 
Def~\ref{eq:def:composite-rewards} only need apply to $\costC$. Call this a macro-cost. Move $k$ into the parenthesis and definition.}

We will apply the preceding with $C=\costC$ and $\gamma=\gamC$ shortly.
But first, a natural use of the composed functions is in defining the
notion of policy evaluation for \psmdps:

\textcolor{red}{This can't take an "atomic cost $C$" because the check-in cost isn't one of these.}


\subsection{The model}


The preceding obviously has an optimal policy too, which we shall denote
$\vect{\pi}^\optc$. Due to the uniform action costs, $\vect{\pi}^\optc$ minimizes
the number of strides needed to move to the goal.

We now have two cost functions, however, we want each cost to be relative to a certain policy. We can do this through \emph{policy evaluation}:
\begin{definition}
\label{def:policy_eval}
Given a \psmdp $\mathcal{M} = \langle S, A, T, C, \gamma, G, \sched \rangle$, a policy $\pi$, and a $k$-composed cost function $C^{k}$, we have the \emph{policy evaluation}
$$ V_\pi(s) = C^{k}(s, \pi(s)) + \gamma \sum_{s' \in S}{T(s', \pi(s), s) V_\pi(s')}
$$
\end{definition}
\textcolor{red}{TODO: ambiguous $\gamma$.}

\textcolor{red}{TODO: Change notation so that stars never go with MDPs; they should denote policies that are execution cost optimal. In fact, better would be
to avoid them all together for this paper.}

Consider
two agents, the \emph{\observer} and the \emph{\actor}, 
who must jointly negotiate a schedule and a policy suiting both their constraints. Operationally, the \observer generates check-ins according to the schedule while the \actor executes the policy. 

The \observer will be interested in some notion of cost for $\sched$, distinct 
from $\costC$.
%It is natural that more frequent check-ins
%involve greater expense to generate, so a measure like the
%following may be intuitive:
%$
%\mathbf{C}_0(\sched) = \lim_{n \to \infty} \frac{1}{n}\sum_{i=0}^{n} \frac{1}{\sched(i)}.
%$
%
%
%One flaw with $\mathbf{C}_0$, however, is that it is oblivious to actual
%execution of a policy using the schedule. Not only is it mismatched with the \actor's model
%(which has discounting to place greater weight earlier, and incurs no cost when the goal is reached),
%but, more importantly, it fails to reflect the task structure---one might 
%expect that more frequent check-ins will yield better performance, but this
%is in fact not always the case (for an example, see \cite[Sect.~III-B]{rossi22periodic}).

Thus, for a schedule, two costs will be of interest for each policy. The first, 
we already have in 
\eqref{eqn:cost-seq-discount}, is
associated closely with the \actor's objectives. But we are
now viewing this more directly as a statement about a given schedule. The
second is for the \observer, but depends upon the \actor's use of the schedule.
%This second cost, can be interpreted as the expected discounted cumulative
%cost in a different \psmdp: 
This second cost, can be interpreted as the expected discounted cumulative
cost using a different cost function: 

\begin{definition}
\label{def:optc}
%Given a \psmdp $\mathcal{M}^\opt = \langle S, A, T, C, \gamma, G, \sched \rangle$, the \emph{check-in} \psmdp $\mathcal{M}^\optc$ has $\langle S, A, T, C_c, \gamma_c, G, \sched \rangle$ with
%\[ C_c^{k,\gamma_c}(s, \vv{a}) = \begin{cases} 
%      0 & s \in G \\
%      1 & s \notin G
%   \end{cases}\textrm{ for all } s \in S, \vv{a} \in A^k.
%\]
A \psmdp $\mathcal{M} = \langle S, A, T, C, \gamma, G, \sched \rangle$ has the $k$-composed $\gamma_c$-discounted \emph{check-in} cost function
\[ C_c^{k,\gamma_c}(s, \vv{a}) = \begin{cases} 
      0 & s \in G \\
      1 & s \notin G
   \end{cases}\textrm{ for all } s \in S, \vv{a} \in A^k.
\]
\end{definition}
\textcolor{red}{
TODO: Point out that $V^\optc_\pi(S_0;\mathcal{M})$ is nothing fancy, just short-hand 
for $V_{\pi}(\InitD;\mathcal{M}^\optc)$ where 
$\mathcal{M}^\optc$ has been obtained from $\mathcal{M}$.
}




As classically, we are interested in optimal policies; the added twist is that
we wish minimizing not just cost of execution (from \costC), but also number of 
required external observations. This is why the previous
pair of definitions, as well as the following one, refer to a generic cost function.

We can now state the problem using both notions of cost:
\begin{definition}  \label{def:dominate}
For some \psmdp $\mathcal{M} = \langle S, A, T, \costC, G, \sched \rangle$, 
initial distribution $\InitD$, then
\begin{enumerate}
\item schedule \sched's \emph{execution cost} is the expected discounted cumulative cost to execute each possible policy, written
 as a function of $\sched$ and $\pi$: 
    \[ \mathbf{E}(\sched, \pi) = V_{\pi^\opt}(\InitD),\]
\item and, schedule \sched's \emph{check-in cost} is the expected discounted number of check-ins until $G$ is 
obtained:
    \[ \mathbf{C}(\sched, \pi) = V_{\pi^\optc}(\InitD) \]
    %\[ \mathbf{C}(\sched, \pi) = \!\! \underset{\scalebox{0.7}{\parbox[l]{34pt}{\centering $s^0\!\sim\!\InitD$\\[-3pt]$\vect{\pi}^\opt$}}\hspace*{22pt}}{\expectation{\idx{\tau}}\!,}\text{where } s^\tau\text{ is the first element in } G.\]
\end{enumerate}
\end{definition}


knew a schedule's costs for every policy, we could compute a Pareto front of policies for that schedule alone. If the Pareto front of $D_2$ dominates the Pareto  front of $D_1$, in that $\forall p_1 \in P(D_1) (\exists p_2 \in P(D_2) (p_2 $ dominates $p_1))$, then $D_2$ dominates $D_1$.


It is infeasible to enumerate every possible policy, so the previous domination criteria must be reduced to fewer policies. If we somehow knew a schedule's costs for every policy, we could compute a Pareto front of policies for that schedule alone. If the Pareto front of $D_2$ dominates the Pareto  front of $D_1$, in that $\forall p_1 \in P(D_1) (\exists p_2 \in P(D_2) (p_2 $ dominates $p_1))$, then $D_2$ dominates $D_1$.
%In order to determine dominance directly as expressed in the previous definition, one would have to determine a schedule's costs for every possible policy. 
%As a given schedule can produce any number of policies, each with different costs, we cannot represent a schedule as a single point on the check-in cost vs. execution cost plot. 
The question thus becomes determining the Pareto front for each schedule.

%The top and right edges of the box form a Pareto front that we call the \emph{realizable front}. No matter what policies exist that we don't know about, we can guarantee that we can produce a policy that beats any policies on or beyond the realizable front, since we have $\pi^\opt$ and $\pi^\optc$. One can interpret the realizable front as an upper bound on the best case scenario.

%On the flip side, consider the bottom left corner of the box. Unlike the realizable front, we have no guarantee that a policy exists in this corner, but we do know it is impossible to produce any policy better than the corner. As such, we call the bottom left front the \emph{optimistic} front, corresponding to a lower bound on the best case scenario. 

%The region bounded by the realizable and optimistic fronts represents uncertainty of the schedule's performance. With just these two policies, $\pi^\opt$ and $\pi^\optc$, we have a box. 


Using this new definition, we can consider a schedule $\sched_1$ dominated by another schedule $\sched_2$ if each point in $\sched_1$'s optimistic front is dominated by some point in $\sched_2$'s realizable front. The interpretation is that all optimal policies in $\sched_1$, even hypothetical ones that may not actually exist, would be worse than a realizable policy in $\sched_2$. This criteria is a looser approximation to the one in Definition~\ref{def:dominate} in that it may produce more non-dominated schedules, but will not incorrectly mark a schedule as dominated.


%\begin{figure}[h]
%    \includegraphics[width=\linewidth]{images/conceptual-1b.pdf}
%    \caption{Example characterization of a schedule.
%    \label{fig:conceptual}}
%\end{figure}
%\begin{figure}[h]
%    \includegraphics[width=\linewidth]{images/conceptual-1b.pdf}
%    \caption{Example characterization of a schedule.
%    \label{fig:conceptual}}
%\end{figure}


%As discussed earlier, we characterize schedules with a realizable front and an optimistic front that bound its performance uncertainty. 

%If we knew the costs for every single possible policy for a schedule, there would be no uncertainty region---the realizable front and the optimistic front would be the same. Such a computation would be absurdly expensive however, if it was even possible.




%\begin{figure}[h]
%    \includegraphics[width=0.8\linewidth]{images/conceptual-2 copy 3.png}
%    \caption{Realizable front (dashed red) and optimistic front (dashed blue) with the introduction of a $\pi^\alpha$ policy (blue circle).
%    \label{fig:conceptual2}}
%\end{figure}

%(a minimization downwards and to the left) 

%Reducing the region of uncertainty provides a more accurate assessment of schedule quality, at the cost of extra computation. However, as we will see later, this extra computation can actually improve performance overall under certain circumstances.

\begin{proposition}[Schedule extension]
Consider a \psmdp for a schedule $\sched$ with value function $U(s)$ and
policy evaluation $V(s)$ for a policy $\pi$. Given a stride $k$ and its \psmdp $\langle S, A, T, C,
\gamma, G, \seq{\recc{k}} \rangle$, the new policy $\pi^\prime$ for the \emph{extended}
schedule $\sched^\prime = \seq{k, \sched(0), \sched(1),\dots}$ has the \emph{extended} value
function $U^\prime(s)$ and \emph{extended} policy evaluation $V^\prime(s)$ as follows:
$$U^\prime(s) = \min_{\vv{a} \in A^k} (C^{k,\gamma}(s, \vv{a}) + \gamma^k \sum_{s^{\prime} \in S} T^k(s', \vv{a}, s) U(s')),$$
$$V^\prime(s) = C^{k,\gamma}(s, \pi^\prime(s)) + \gamma^k \sum_{s^{\prime} \in S} T^k(s', \pi^\prime(s), s) V(s').$$
\end{proposition}



